Probabilistic Value Selection for Space Efficient Model

An alternative to current mainstream preprocessing methods is proposed: Value Selection (VS). Unlike the existing methods such as feature selection that removes features and instance selection that eliminates instances, value selection eliminates the values (with respect to each feature) in the dataset with two purposes: reducing the model size and preserving its accuracy. Two probabilistic methods based on information theory's metric are proposed: PVS and P + VS. Extensive experiments on the benchmark datasets with various sizes are elaborated. Those results are compared with the existing preprocessing methods such as feature selection, feature transformation, and instance selection methods. Experiment results show that value selection can achieve the balance between accuracy and model size reduction.

==> meta/author_ieee_blank.tex <==
\author{\IEEEauthorblockN{Author1, Author2, Author3, Author4}
\IEEEauthorblockA{\textit{Sub-affiliation} \\
\textit{Affiliation}\\
Country \\
email1, email2, email3, email4}
}

==> sections/0_keyword.tex <==
\begin{keyword}
preprocessing
\sep data mining
\sep value selection
\sep model size reduction
\sep entropy
\sep information gain
% \sep probabilistic approach
% \sep decision tree
%% keywords here, in the form: keyword \sep keyword

%% MSC codes here, in the form: \MSC code \sep code
%% or \MSC[2008] code \sep code (2000 is the default)

\end{keyword}

==> sections/6_discussions.tex <==
\newcommand{\pendigits}{\textit{pendigits}}
\newcommand{\Pendigits}{\textit{Pendigits}}
\section{Case Study: \Pendigits{} dataset}
\label{sec:fvs:case}
% \newcommand{\adult}{\textit{adult}}
% \newcommand{\Adult}{\textit{Adult}}
% \newcommand{\dota}{\textit{dota2}}
% \newcommand{\Dota}{\textit{Dota2}}
% Case studies of \fvs performances
Exploring the data distribution changes after the preprocessing could help to provide more insights on how it works. 
% Particularly, two datasets with different characteristics are discussed in this section: \pendigits{} and \dota{}. Both \Pendigits{} and \dota{} datasets do not have missing values so the missing values exist only caused by \fvs{} process. In terms of size, \dota{} is larger than \pendigits{} dataset. In terms of class label, binary classification is solved in \dota{} dataset while multi class problem is dealt in \pendigits{}. 
In particular, \pendigits{} dataset is used in this case study because of the following reasons. \Pendigits{} dataset do not have missing values so the only reason missing values are observed in the data is because of the \fvs{} process. Also, the number of feature and instance are moderate so it can be observed clearly as a case study but it does not hinder the observation to be scaled to a larger problem. Finally, the multi class problem dealt in \pendigits{} presents another challenge to the preprocessing methods.
The baselines compared in this case study are limited to best performer in each category: Reservoir instance selection \cite{Vitter:1985:RSR:3147.3165}, PCA feature transformation \cite{pearson1901liii}, and Correlation feature selection \cite{Hall1998}. To evaluate the effectiveness of each method, the classification used for evaluation is Decision Tree \cite{Quinlan:1993:CPM:152181} and a rule-based method called Ripper \cite{Cohen:1995:FER:3091622.3091637}.

\begin{figure*}
    \centering
    \subfigure[Original]{\label{fig:fvs:casestudy:case2:dist:original}\includegraphics[width=0.48\textwidth]{figures/case2/case2_dist_ori.png}} \hspace{6pt}
    \subfigure[\Fvs]{\label{fig:fvs:casestudy:case2:dist:fvs}\includegraphics[width=0.48\textwidth]{figures/case2/case2_dist_fvs.png}}
    \subfigure[Reservoir]{\label{fig:fvs:casestudy:case2:dist:reservoir}\includegraphics[width=0.48\textwidth]{figures/case2/case2_dist_reservoir.png}} \hspace{6pt}
    \subfigure[CFS]{\label{fig:fvs:casestudy:case2:dist:cfs}\includegraphics[width=0.48\textwidth]{figures/case2/case2_dist_cfs.png}}
    \subfigure[PCA]{\label{fig:fvs:casestudy:case2:dist:pca}\includegraphics[width=0.48\textwidth]{figures/case2/case2_dist_pca.png}}
	\caption{Data distribution of \pendigits{} dataset provided after each preprocessing: (a) original dataset, (b) \fvs{}, (c) Reservoir instance selection, (d) Correlation feature selection, (e) PCA feature transformation.}
	\label{fig:fvs:distribution}
\end{figure*}

\begin{table}[h]
\centering
\caption{Performance comparisons on each preprocessing method in the \pendigits{} dataset.}
\label{tab:fvs:case2}
\begin{small}
\begin{tabular}{l|cccc}
\hline
Preprocessing & Accuracy (Tree) & Model Size (Tree) & Accuracy (Rules) & Model Size (Rules) \\ \hline
None (original) & 88.3\% & 1981 & 90.9\% & 223 \\
\Fvs & 79.8\% & 991 & 81.6\% & 134 \\
Reservoir & 67.5\% & 211 & 71.3\% & 39 \\
PCA & 86.4\% & 873 & 84.3\% & 102 \\
CFS & 87.5\% & 1941 & 90.7\% & 219 \\
Removing columns & 84.4\% & 1721 & 84.5\% & 192 \\ \hline
\end{tabular}
\end{small}
\end{table}

\begin{figure*}
    \centering
    \subfigure[Original]{\label{fig:fvs:casestudy:case2:tree:original}\includegraphics[width=0.85\textwidth]{figures/case2/case2_tree_ori.png}}
    \subfigure[\Fvs{}]{\label{fig:fvs:casestudy:case2:tree:fvs}\includegraphics[width=0.85\textwidth]{figures/case2/case2_tree_fvs.png}}
    \subfigure[Reservoir]{\label{fig:fvs:casestudy:case2:tree:reservoir}\includegraphics[width=0.85\textwidth]{figures/case2/case2_tree_reservoir.png}}
    \subfigure[CFS]{\label{fig:fvs:casestudy:case2:tree:cfs}\includegraphics[width=0.85\textwidth]{figures/case2/case2_tree_cfs.png}}
    \subfigure[PCA]{\label{fig:fvs:casestudy:case2:tree:pca}\includegraphics[width=0.85\textwidth]{figures/case2/case2_tree_pca.png}}
	\caption{Decision tree built based on the data provided by each preprocessing: (a) original dataset, (b) \fvs{}, (c) Reservoir instance selection, (d) Correlation feature selection, (e) PCA feature transformation. Circle shaped objects are internal node and square shaped objects are leaves.}
	\label{fig:fvs:casetree}
\end{figure*}

\begin{table}[h]
\caption{Top-10 Rules produced on each preprocessing method (except PCA) in the \pendigits{} dataset.}
\centering
\label{tab:fvs:rules}
\begin{scriptsize}
\begin{tabular}{l}
\hline
\textbf{Original} \\ \hline
(input13 = '(90-inf)') and (input8 = '(-inf-10{]}') and (input9 = '(-inf-10{]}') =\textgreater class=8 \\
(input16 = '(80-90{]}') and (input4 = '(90-inf)') and (input11 = '(-inf-10{]}') =\textgreater class=8 \\
(input16 = '(70-80{]}') and (input4 = '(90-inf)') and (input11 = '(-inf-10{]}') =\textgreater class=8 \\
(input16 = '(90-inf)') and (input4 = '(90-inf)') and (input11 = '(-inf-10{]}') =\textgreater class=8 \\
(input13 = '(90-inf)') and (input14 = '(90-inf)') =\textgreater class=8 \\
(input16 = '(80-90{]}') and (input5 = '(90-inf)') =\textgreater class=8 \\
(input16 = '(70-80{]}') and (input4 = '(90-inf)') and (input6 = '(70-80{]}') =\textgreater class=8 \\
(input16 = '(70-80{]}') and (input5 = '(90-inf)') =\textgreater class=8 \\
(input10 = '(-inf-10{]}') and (input7 = '(90-inf)') and (input3 = '(-inf-10{]}') and (input4 = '(80-90{]}') =\textgreater class=8 \\
(input16 = '(60-70{]}') and (input11 = '(-inf-10{]}') =\textgreater class=8 \\
\hline
\textbf{\Fvs{}} \\ \hline
(input16 = '(90-inf)') and (input11 = '(-inf-10{]}') =\textgreater class=8 \\
(input16 = '(90-inf)') and (input11 = '(50-60{]}') =\textgreater class=8 \\
(input16 = '(90-inf)') and (input11 = '(40-50{]}') =\textgreater class=8 \\
(input16 = '(70-80{]}') and (input10 = '(-inf-10{]}') =\textgreater class=8 \\
(input16 = '(80-90{]}') and (input11 = '(-inf-10{]}') and (input10 = '(-inf-10{]}') =\textgreater class=8 \\
(input14 = '(90-inf)') and (input12 = '(60-70{]}') and (input10 = '(30-40{]}') =\textgreater class=8 \\
(input16 = '(90-inf)') and (input11 = '(30-40{]}') =\textgreater class=8 \\
(input14 = '(90-inf)') and (input5 = '(90-inf)') =\textgreater class=8 \\
(input16 = '(90-inf)') and (input11 = '(20-30{]}') =\textgreater class=8 \\
(input14 = '(90-inf)') and (input5 = '(60-70{]}') =\textgreater class=8 \\
\hline
\textbf{Reservoir} \\ \hline
(input10 = '(-inf-10{]}') =\textgreater class=8 \\
(input13 = '(90-inf)') and (input14 = '(90-inf)') =\textgreater class=8 \\
(input12 = '(-inf-10{]}') =\textgreater class=8 \\
(input5 = '(90-inf)') and (input8 = '(-inf-10{]}') =\textgreater class=8 \\
\hline
\textbf{CFS} \\ \hline
(input16 = '(90-inf)') and (input9 = '(-inf-10{]}') =\textgreater class=8 \\
(input16 = '(80-90{]}') and (input4 = '(90-inf)') =\textgreater class=8 \\
(input16 = '(70-80{]}') and (input10 = '(-inf-10{]}') and (input11 = '(-inf-10{]}') =\textgreater class=8 \\
(input16 = '(90-inf)') and (input4 = '(90-inf)') and (input11 = '(-inf-10{]}') =\textgreater class=8 \\
(input14 = '(90-inf)') and (input7 = '(-inf-10{]}') =\textgreater class=8 \\
(input16 = '(90-inf)') and (input7 = '(90-inf)') and (input4 = '(80-90{]}') =\textgreater class=8 \\
(input8 = '(-inf-10{]}') and (input5 = '(90-inf)') =\textgreater class=8 \\
(input16 = '(80-90{]}') and (input9 = '(10-20{]}') =\textgreater class=8 \\
(input16 = '(90-inf)') and (input9 = '(10-20{]}') =\textgreater class=8 \\
(input16 = '(70-80{]}') and (input4 = '(90-inf)') =\textgreater class=8 \\ \hline
\end{tabular}
\end{scriptsize}
\end{table}

% \textbf{\Pendigits{} dataset.}
Firstly, Figure \ref{fig:fvs:casestudy:case2:dist:original} shows the data distribution of the original \pendigits{} dataset using equal-width (Binning) discretization. The last column represents the 10 class labels and each color reflects each class label given in each feature. Followings are the data distribution on each preprocessing method. 

The data distribution after applying \fvs{} is shown in Figure \ref{fig:fvs:casestudy:case2:dist:fvs}. It is interesting to see that a few attributes (i.e., input2, input3, input4, input6, input7, input8, input9, and input13) do not have data distribution. This result represents how the \fvs{} act as a feature selection. However, the results given by removing all the columns suggested in Figure \ref{fig:fvs:casestudy:case2:dist:fvs} does not produce the same result as the \fvs{}; in fact, the result of removing these columns do not reduce the model size significantly, as shown in Table \ref{tab:fvs:case2}. This explains the differences between the proposed \fvs{} and feature selection method: \fvs{} not only able to remove features but also instances and values. Reservoir instance selection produces similar data distribution to the original data except it has fewer samples as shown in Figure \ref{fig:fvs:casestudy:case2:dist:reservoir}. Correlation feature selection removes 3 features (i.e., input6, input12, input13) that is deemed as irrelevant features, as shown in \ref{fig:fvs:casestudy:case2:dist:cfs}. Finally, the data distribution post PCA processing is shown in Figure \ref{fig:fvs:casestudy:case2:dist:pca}. The data is transformed into another data space whose number of attribute is half of the original dataset. As the data is transformed to different space, the data distribution is considerably different than the other preprocessing methods and the original data.

Looking deeper into the tree built by each preprocessing, Figure \ref{fig:fvs:casetree} presents an interesting insight. Firstly, Reservoir instance selection reduces the complexity of the tree significantly, as shown in Figure \ref{fig:fvs:casestudy:case2:tree:reservoir}. On the other hand, the proposed \fvs{} method reduce the complexity of tree moderately by trimming some insignificant branches and leaves. The CFS cannot reduce the complexity of the tree significantly, as shown in Figure \ref{fig:fvs:casestudy:case2:tree:cfs}. The reason that CFS maintain complex tree structure is because it prioritizes accuracy than reducing model complexity. Finally, the tree built by PCA has substantial differences compared to the other trees: excessive number of internal nodes and broader tree with shallower depth.

The rules generated in each preprocessing are also interesting to be studied. Each preprocessing method prioritize specific class label in their rules. For example, in the original data, class label "8" is put in the top of the list while in \fvs{} prioritize class label "3". Similarly, Reservoir instance selection, CFS, and PCA arrange the class label "6", "5", and "9" to occupy the top initial rules in the list, respectively. To study the rules used to depict a class label, Table \ref{tab:fvs:rules} lists the top-10 rules used to determine class label "8"\footnote{Please note that the class label for the study is arbitrarily selected since the distribution of each class is similar.}. Here, PCA's rules are not compared in this study as the features used in PCA are transformed into a different space. The observation on the rules are explained as follows. 
The first rule in the \fvs{} method is similar to the second rule in the original data, except that "input4" is not considered in \fvs{} method. The rules in Reservoir instance selection seems to be oversimplified by considering one or two features in each rule. Rules built after the CFS is significantly different to the original model yet it could maintain similar accuracy performance. The conclusion of the above observation is that each preprocessing prioritize specific aspect of the data and it is simply the bias and variance trade-off.

% \begin{figure*}
%     \centering
%     \subfigure[Original]{\label{fig:fvs:casestudy:case3:dist:original}\includegraphics[width=0.3\textwidth]{figures/case/case3_dist_ori.png}} \hspace{6pt}
%     \subfigure[\Fvs]{\label{fig:fvs:casestudy:case3:dist:fvs}\includegraphics[width=0.3\textwidth]{figures/case/case3_dist_fvs.png}} \hspace{6pt}
%     \subfigure[Reservoir]{\label{fig:fvs:casestudy:case3:dist:reservoir}\includegraphics[width=0.3\textwidth]{figures/case/case3_dist_reservoir.png}}
%     \subfigure[CFS]{\label{fig:fvs:casestudy:case3:dist:cfs}\includegraphics[width=0.3\textwidth]{figures/case/case3_dist_cfs.png}} \hspace{6pt}
%     \subfigure[PCA]{\label{fig:fvs:casestudy:case3:dist:pca}\includegraphics[width=0.3\textwidth]{figures/case/case3_dist_pca.png}}
% 	\label{fig:fvs:casestudy:case3:distribution}
% 	\caption{Data distribution on \dota{} dataset provided after each preprocessing: (a) original dataset, (b) \fvs{}, (c) Reservoir instance selection, (d) Correlation feature selection, (e) PCA feature transformation.}
% \end{figure*}

% \subsection{\Dota{} dataset}
% The original data distribution of \dota{} dataset on MDL discretization \cite{Fayyad1993,Kononenko1995} is presented in Figure \ref{fig:fvs:casestudy:case3:dist:original}. The reason of evaluating this dataset on MDL discretization is because the data is not distributed evenly and MDL discretization is known to be able to select the best cut on the data based on the information gain. Also, the figure only shows the first 40 attributes due to the excessive amount of feature in \dota{} dataset.
